Composable Model-Free RL for Navigation with Input-Affine Systems

As autonomous robots move into complex, dynamic real-world environments, they must learn to navigate safely in real time, yet anticipating all possible behaviors is infeasible. We propose a composable, model-free reinforcement learning method that learns a value function and an optimal policy for each individual environment element (e.g., goal or obstacle) and composes them online to achieve goal reaching and collision avoidance. Assuming unknown nonlinear dynamics that evolve in continuous time and are input-affine, we derive a continuous-time Hamilton-Jacobi-Bellman (HJB) equation for the value function and show that the corresponding advantage function is quadratic in the action and optimal policy. Based on this structure, we introduce a model-free actor-critic algorithm that learns policies and value functions for static or moving obstacles using gradient descent. We then compose multiple reach/avoid models via a quadratically constrained quadratic program (QCQP), yielding formal obstacle-avoidance guarantees in terms of value-function level sets, providing a model-free alternative to CLF/CBF-based controllers. Simulations demonstrate improved performance over a PPO baseline applied to a discrete-time approximation.

==> preamble/math.tex <==
% AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
  \usepackage{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
  \usepackage{amsthm}%
}{}
\makeatother
% Generic symbols (e.g., \degree)
\usepackage{gensymb}
% Prescripts, squashed summations, and others
\usepackage{mathtools}
% Bold greek letters
\usepackage{bm}

% Extend amsthm \newtheorem to include continued version
\usepackage{refcount}
\newcommand{\newtheoremcontinued}[2]{%
  % create environment
  \newtheorem{#1}{#2}
  % counter to copy counter number
  \newcounter{#1previous}
  % define continued version of the environment
  \NewDocumentEnvironment{#1continued}{O{Continued} m}
  {
    % store current counter
    \setcounter{#1previous}{\value{#1}}%
    % set it to number extracted from reference
    \edef\tempcount#1{\getrefnumber{##2}}%
    \setcounter{#1}{\tempcount#1}%
    % amsthm will increase this value by one, so we compensate
    \addtocounter{#1}{-1}
    % Begin amsthm environment
    \begin{#1}[##1]
    }
    {
    \end{#1}
    % restore original counter value
    \setcounter{#1}{\value{#1previous}}%
  }
}


% Common math statements environments
\makeatletter
\@ifundefined{theorem}{
  \newtheoremcontinued{theorem}{Theorem}
  \newtheoremcontinued{corollary}{Corollary}
  \newtheoremcontinued{proposition}{Proposition}
  \newtheoremcontinued{lemma}{Lemma}
  \newtheoremcontinued{fact}{Fact}
  \newtheoremcontinued{problem}{Problem}
  \newtheoremcontinued{assumption}{Assumption}
  \newtheoremcontinued{property}{Property}
  \newtheoremcontinued{remark}{Remark}
  \newtheoremcontinued{example}{Example}
}{}
% SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{%
  \newtheoremcontinued{definition}{Definition}%
}
% \@ifundefined{remark}{
%   \newtheoremcontinued{remark}{Remark}
% }
\makeatother
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables:
%%% mode: latex
%%% End:

